AC-Informed DC Optimal Transmission Switching Problems via Parameter Optimization

Optimal Transmission Switching (OTS) problems minimize operational costs while treating both the transmission line energization statuses and generator setpoints as decision variables. The combination of nonlinearities from an AC power flow model and discrete variables associated with line statuses makes AC-OTS a computationally challenging Mixed-Integer Nonlinear Program (MINLP). To address these challenges, the DC power flow approximation is often used to obtain a DC-OTS formulation expressed as a Mixed-Integer Linear Program (MILP). However, this approximation often leads to suboptimal or infeasible switching decisions when evaluated with an AC power flow model. This paper proposes an enhanced DC-OTS formulation that leverages techniques for training machine learning models to optimize the DC power flow model's parameters. By optimally selecting parameter values that align flows in the DC power flow model with apparent power flows -- incorporating both real and reactive components -- from AC Optimal Power Flow (OPF) solutions, our method more accurately captures line congestion behavior. Integrating these optimized parameters into the DC-OTS formulation significantly improves the accuracy of switching decisions and reduces discrepancies between DC-OTS and AC-OTS solutions. We compare our optimized DC-OTS model against traditional OTS approaches, including DC-OTS, Linear Programming AC (LPAC)-OTS, and Quadratic Convex (QC)-OTS. Numerical results show that switching decisions from our model yield better performance when evaluated using an AC power flow model, with up to $44\%$ cost reductions in some cases.

==> text/OTS.tex <==
\section{Application to OTS}
\label{sec:OTS}
Expanding upon the DCOPF model detailed in Model \ref{model:DCOPF_matrixformat}, the DC-OTS model (Model \ref{model:DCOPFOTS_matrixformat}) \cite{fisher2008optimal, hedman2008optimal, hedman2009optimal} enhances power system optimization by considering not only generation costs but also configurations of transmission lines. This is facilitated through the integration of a binary variable $\mathbf{u}$, which indicates the operational status of each transmission line, either active (closed) or inactive (open).

In this enhanced model, the binary variable $\mathbf{u}$ determines whether a line is operational, influencing the dispatch cost by potentially removing a line from the network. This modification can result in scenarios where no lines are deactivated, leaving the objective function unchanged, or where one or more lines are deactivated, potentially improving the objective function value.

The core elements such as the objective function (\ref{eq:DCOPFOTS:obj_matrixformat}), generator output constraints (\ref{eq:DCOPFOTS:bounds:pg_matrixformat}), and the power balance (\ref{eq:DCOPFOTS:power_balance_matrixformat}) remain consistent with those defined in the original DCOPF model (\ref{model:DCOPF_matrixformat}). Adjustments to account for the operational status of transmission lines are made in (\ref{eq:DCOPFOTS:powerflow_matrixformat}), where the line capacities $\overline{\mathbf{S}}$ are effectively nullified by setting $\mathbf{u}$ to zero, thus preventing any power flow through deactivated lines.
%
The 'big-M' method, detailed in (\ref{eq:DCOPFOTS:bounds:pf_matrixformat1}) and (\ref{eq:DCOPFOTS:bounds:pf_matrixformat2}), utilizes large numeric values to ensure constraints are satisfied independently of bus angle discrepancies when lines are inactive. This approach prevents any forced angle equalization across buses connected by non-operational lines, maintaining accurate modeling even when lines are removed, such as in scenarios involving parallel transmission elements.
%
The voltage angle at the reference bus is fixed at zero (\ref{eq:DCOPFOTS:theta_ref}), and voltage angle limits imposed by (\ref{eq:DCOPFOTS:theta}).
%
Finally, the model imposes a limit on the number of lines that can be deactivated (i.e, $\Omega$) (\ref{eq:DCOPFOTS:switch}), allowing for strategic modifications to the transmission network's configuration, thus facilitating an exploration of different network topologies and their impacts on system performance.







\begin{model}[!t]
    \caption{The DC-OTS Problem}
    \label{model:DCOPFOTS_matrixformat}
    \begin{subequations}
    \label{eq:DCOPFOTS_matrixformat}
    \normalsize
    \begin{align}
       \min_{\mathbf{p}^{\text{g}} , \boldsymbol{\theta}, \mathbf{z}} \quad 
        & {\mathbf{p}^{\text{g}}}^{\top}\text{diag}(\mathbf{c}_{2}) \mathbf{p}^{\text{g}}+ \mathbf{c}^{\top}_{1}\mathbf{p}^{\text{g}} + \sum_{i \in \mathcal{N}}c_{0i}  + c^{profit}\mathbf{1}^{\top}(\mathbf{1}-\mathbf{u})\label{eq:DCOPFOTS:obj_matrixformat}\\
        \text{s.t.} \quad \nonumber\\
         & \underline{\textbf{p}}^{\text{g}} \leq \mathbf{p}^{\text{g}} \leq \overline{\textbf{p}}^{\text{g}}
               \label{eq:DCOPFOTS:bounds:pg_matrixformat}\\
            &  \mathbf{p}^{\text{g}} - \textbf{p}^{\text{d}} - {\boldsymbol{\gamma}} = \mathbf{A}^{\top}\boldsymbol{p}^{flow}    
               \label{eq:DCOPFOTS:power_balance_matrixformat}\\
               &|\boldsymbol{p}^{flow}| \leq {\mathbf{u} } \circ \overline{\mathbf{S}} 
                       \label{eq:DCOPFOTS:powerflow_matrixformat}\\
            & \text{diag}(\mathbf{b})\mathbf{A}  \boldsymbol{\theta} 
            +{\boldsymbol{\rho}}+ (\mathbf{1}- {\mathbf{u})}\circ \mathbf{M}\geq \boldsymbol{p}^{flow} 
                \label{eq:DCOPFOTS:bounds:pf_matrixformat1}\\ 
            & \text{diag}(\mathbf{b})\mathbf{A} \boldsymbol{\theta}+{\boldsymbol{\rho}} - (\mathbf{1}- {\mathbf{u}})\circ \mathbf{M}\leq \boldsymbol{p}^{flow} 
            \label{eq:DCOPFOTS:bounds:pf_matrixformat2}\\ 
            & \theta_{\text{ref}} = 0 \label{eq:DCOPFOTS:theta_ref}\\
            %& \underline{\boldsymbol{\theta}} \leq \boldsymbol{\theta} \leq \overline{\boldsymbol{\theta}}
            %   \label{eq:DCOPFOTS:theta}\\
            %& (\mathbf{1}-\mathbf{u})\mathbf{1}^{\top} \leq \Omega
            %\label{eq:DCOPFOTS:switch}\\
            & \mathbf{u} \in \{0,1\}^{|L|}
                \label{eq:DCOPFOTS:z_binary}
    \end{align}
    \end{subequations}
\end{model}








% Building on top of the DCOPF model shown in Model \ref{model:DCOPF_matrixformat} the DCOPF-OTS model (Model \ref{model:DCOPFOTS_matrixformat}) \cite{fisher2008optimal, hedman2008optimal, hedman2009optimal} aims to optimize the power system's operation by considering both generation costs and transmission line configurations by including the binary variable $\mathbf{u}$ as the status of the switch of the transmission lines. 
% %
% In this new formulation, each line is assigned a binary variable,$\mathbf{u}$, that represents whether the line is included in the system (the circuit breaker on that line is closed) or not (circuit breaker is open). Because of the peculiar characteristics of electricity, it is possible to improve the dispatch cost by removing a
% line from the network. Thus the optimization problem will either return the result that no lines are taken out with no change in the objective function value, or that one or more lines are opened with an improved objective function.


% The objective function (\ref{eq:DCOPFOTS:obj_matrixformat}), generator output limits \eqref{eq:DCOPFOTS:bounds:pg_matrixformat}, and power balance \eqref{eq:DCOPFOTS:power_balance_matrixformat} are the same as \eqref{eq:DCOPF:obj_matrixformat}, \eqref{eq:DCOPF:bounds:pg_matrixformat}, and \eqref{eq:DCOPF:power_balance_matrixformat} from Model \ref{model:DCOPF_matrixformat}. 
% %
% Thermal limits on transmission lines are imposed by \eqref{eq:DCOPFOTS:powerflow_matrixformat}, where the capacity of the lines $\overline{\mathbf{S}}$ is multiplied by the lines' switch status $\mathbf{u}$ so that power flow of the lines $\mathbf{p}^{flow}$ is zero when $\mathbf{u}$ is zero.
% %
% $\mathbf{M}$, listed in \eqref{eq:DCOPFOTS:bounds:pf_matrixformat1} and \eqref{eq:DCOPFOTS:bounds:pf_matrixformat2}, is refered as the "big-M" values. When the binary variable $\mathbf{u}$ is equal to one, the value of $M$ does not matter; when the binary variable $\mathbf{u}$ is equal to zero, the value of $\mathbf{M}$ is used to ensure that \eqref{eq:DCOPFOTS:bounds:pf_matrixformat1} and \eqref{eq:DCOPFOTS:bounds:pf_matrixformat2} are satisfied regardless of the difference in the bus angles. 
% $\mathbf{p}^{flow}$ is zero when $\mathbf{u}$ is zero so for this to work. $\mathbf{M}$ must be a large number greater than ${\text{diag}(\mathbf{b})\mathbf{A}\boldsymbol{\theta}}^{max}$. Without this adjustment to the power flow equations, the buses that are connected to this transmission element would be forced to have the same bus angle when $\mathbf{u}$ is zero.
% %
% Forcing the buses’ angles to be the same is incorrect as the element is no longer present. For the situation where there are two parallel transmission elements, if one were removed by the program, the other would be forced to have a zero power flow without this adjustment to the power flow equations. However, using \eqref{eq:DCOPFOTS:bounds:pf_matrixformat1} and \eqref{eq:DCOPFOTS:bounds:pf_matrixformat2}, the DCOPF provides the solution corresponding to the case when the opened transmission element is not present in the network.
% %
% Analogous to \eqref{eq:DCOPF:theta-ref_matrixformat}, the voltage angle at reference bus \eqref{eq:DCOPFOTS:theta_ref} is set to zero. The voltage angles at the buses are constrained \eqref{eq:DCOPFOTS:theta} within predefined limits\footnote{Upper and lower voltage angle constraints were set to $0.6$ and $-0.6$ radians, respectively. While these bounds are conservative, they aid in finding solutions in a timely manner. Loosening these bounds may result in improved solutions}. 
% %
% Finally, \eqref{eq:DCOPFOTS:switch} imposes the maximum number of lines that can be opened to alter the configuration of the transmission network.
% %


